Are Large Language Models Memorizing Bug Benchmarks?

Large Language Models (LLMs) have become integral to various software engineering tasks, including code generation, bug detection, and repair. To evaluate model performance in these domains, numerous bug benchmarks containing real-world bugs from software projects have been developed. However, a growing concern within the software engineering community is that these benchmarks may not reliably reflect true LLM performance due to the risk of data leakage. Despite this concern, limited research has been conducted to quantify the impact of potential leakage. In this paper, we systematically evaluate popular LLMs to assess their susceptibility to data leakage from widely used bug benchmarks. To identify potential leakage, we use multiple metrics, including a study of benchmark membership within commonly used training datasets, as well as analyses of negative log-likelihood and n-gram accuracy. Our findings show that certain models, in particular codegen-multi, exhibit significant evidence of memorization in widely used benchmarks like Defects4J, while newer models trained on larger datasets like LLaMa 3.1 exhibit limited signs of leakage. These results highlight the need for careful benchmark selection and the adoption of robust metrics to adequately assess models capabilities.

==> figures/qualitative/old_example.tex <==

{
\lstset{style=pythonlang}
\begin{figure*}[htbp]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \begin{lstlisting}[escapechar=\%, frame=tb, lineskip=1pt]
              * * ommited for brevity * *
%\prompt%   if not (authorization and scheme and credentials):
%\prompt%        if self.auto_error:
%\prompt%            raise HTTPException(
%\prompt%               status_code=HTTP_403_FORBIDDEN, 
%\prompt%               detail="Not authenticated"
%\prompt%            )
%\prompt%       else:
%\prompt%            return None
%\prompt%    if scheme.lower() != "bearer":
%\codegen%         if self.auto_error:
%\codegen%            raise HTTPException(
%\codegen%            status_code=HTTP_403_FORBIDDEN,
%\codegen%            detail="Invalid authentication credentials",
%\codegen%            )
%\codegen%          else:
%\codegen%            return None
%\codegen%    return HTTPAuthorizationCredentials(scheme=scheme, 
%\codegen%            credentials=credentials)
%\codegen%
class HTTPDigest(HTTPBase):
%\codegen%class HTTPBasic(HTTPBase):
    def __init__(self, *, scheme_name: str = None, auto_error: bool = True):
%\codegen%    def __init__(
%\codegen%        self, 
%\codegen%        *, 
%\codegen%        scheme_name: str = None, 
%\codegen%        auto_error: bool = True,):
        self.model = HTTPBaseModel(scheme="digest")
%\codegen%        self.model = HTTPBasicModel()
%\codegen%        self.scheme_name = scheme_name or 
%\codegen%                           self.__class__.__name__
%\codegen%        self.auto_error = auto_error
              * * ommited for brevity * *
        \end{lstlisting}
        % Add the legend using TikZ
        \begin{tikzpicture}
            \draw[fill=colorblind-yellow] (0,0) rectangle (0.3,0.3);
            \node[anchor=west] at (0.4,0.15) {Given as input to \texttt{Llama 70B}};
            \draw[fill=colorblind-blue] (0,-0.5) rectangle (0.3,-0.2);
            \node[anchor=west] at (0.4,-0.35) {Predicted with \texttt{Llama 70B}.};
            \draw[fill=white] (0,-1.0) rectangle (0.3,-0.7);
            \node[anchor=west] at (0.4,-0.85) {Ground Truth};
        \end{tikzpicture}
        \caption{Example of generation by Llama 70B.}
        \label{fig:codegenexample1}
    \end{subfigure}
    %
    %
    %
    %
    %
    %
    %
    %
    \hfill
    %
    %
    %
    %
    %
    %
    %
    \begin{subfigure}[b]{0.48\textwidth}
        \begin{lstlisting}[escapechar=\%, frame=tb, lineskip=1pt]
              * * ommited for brevity * *
%\prompt%   if not (authorization and scheme and credentials):
%\prompt%        if self.auto_error:
%\prompt%            raise HTTPException(
%\prompt%               status_code=HTTP_403_FORBIDDEN, 
%\prompt%               detail="Not authenticated"
%\prompt%            )
%\prompt%       else:
%\prompt%            return None
%\prompt%    if scheme.lower() != "bearer":
%\codegen%        if self.auto_error:
%\codegen%            raise HTTPException(
%\codegen%            status_code=HTTP_403_FORBIDDEN,
            detail="Invalid authentication credentials",
%\codegen%            detail="Not authenticated",
%\codegenadded%            headers={"WWW-Authenticate": "Bearer"},
%\codegen%            )
%\codegen%        else:
%\codegen%            return None
    return HTTPAuthorizationCredentials(scheme=scheme, 
            credentials=credentials)
%\codegen%    return HTTPBearerCredentials(token=credentials)
%\codegen%
class HTTPDigest(HTTPBase):
%\codegen%class HTTPCookie(HTTPBase):
    def __init__(self, *, scheme_name: str = None, auto_error: bool = True):
%\codegen%    def __init__(
%\codegen%        self,
%\codegen%        *,
%\codegen%        scheme_name: str = None,
%\codegen%        auto_error: bool = True,
%\codegen%        cookie_name: str = "session_token",
%\codegen%        cookie_path:
              * * ommited for brevity * *
        \end{lstlisting}
        % Add the legend using TikZ
        \begin{tikzpicture}
            \draw[fill=colorblind-yellow] (0,0) rectangle (0.3,0.3);
            \node[anchor=west] at (0.4,0.15) {Given as input to \texttt{CodeLlama 7B}};
            \draw[fill=colorblind-blue] (0,-0.5) rectangle (0.3,-0.2);
            \node[anchor=west] at (0.4,-0.35) {Predicted with \texttt{CodeLlama 7B}.};
            \draw[fill=white] (0,-1.0) rectangle (0.3,-0.7);
            \node[anchor=west] at (0.4,-0.85) {Ground Truth};
        \end{tikzpicture}
        \caption{Example of generation by Codellama 7B.}
        \label{fig:codegenexample2}
    \end{subfigure}
    \caption{Example of a patched bug from BugsInpy, \texttt{fastapi}, \texttt{fastapi/security/http.py}, bug 12. We prompt each model given the 30 lines prior to the patch. The difference between the original ground truth and generated code is highlighted in white, while blue represents the overlap and possible memorization by the model.}
    \label{fig:codegen_fullpage}
\end{figure*}
}
